Algorithmic Obfuscation over GF($2^m$)

Galois Field arithmetic blocks are the key components in many security applications, such as Elliptic Curve Cryptography (ECC) and the S-Boxes of the Advanced Encryption Standard (AES) cipher. This paper introduces a novel hardware intellectual property (IP) protection technique by obfuscating arithmetic functions over Galois Field (GF), specifically, focusing on obfuscation of GF multiplication that underpins complex GF arithmetic and elliptic curve point arithmetic functions. Obfuscating GF multiplication circuits is important because the choice of irreducible polynomials in GF multiplication has the great impact on the performance of the hardware designs, and because the significant effort is spent on finding an optimum irreducible polynomial for a given field, which can provide one company a competitive advantage over another.

==> 4-bit-p_x_comparison.tex <==
\begin{figure}[!htb]
\centering
%\caption{My caption}
\begin{tabular}{lllllll}
     &      &      & $a_3$   & $a_2$   & $a_1$   & $a_0$   \\
     &      &      & $b_3$   & $b_2$   & $b_1$   & $b_0$   \\ \hline
     &      &      & $a_{3}b_{0}$ & $a_{2}b_{0}$ & $a_{1}b_{0}$ & $a_{0}b_{0}$ \\
     &      & $a_{3}b_{1}$ & $a_{2}b_{1}$ & $a_{1}b_{1}$ & $a_{0}b_{1}$ &  \\
     & $a_{3}b_{2}$ & $a_{2}b_{2}$ & $a_{1}b_{2}$ & $a_{0}b_{2}$  &      &      \\
$a_{3}b_{3}$ & $a_{2}b_{3}$ & $a_{1}b_{3}$ & $a_{0}b_{3}$  &      &      &      \\ \hline
$s_6$   & $s_5$   & $s_4$   & $s_3$   & $s_2$   & $s_1$   & $s_0$  \\
\end{tabular}
\vspace{2mm}
        \begin{minipage}{.5\linewidth}
      %\caption{$P(x)$=$x^{4}+x^{3}+1$}
      \centering
\begin{tabular}{cccc}
\multicolumn{4}{l}{$P(x)$=$x^{4}+x^{3}+1$}                                                                            \\
\multicolumn{1}{c|}{$s_3$} & \multicolumn{1}{c|}{$s_2$} & \multicolumn{1}{c|}{$s_1$} & $s_0$                     \\
\multicolumn{1}{c|}{$s_4$} & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{0} & $s_4$                     \\
\multicolumn{1}{c|}{$s_5$} & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{$s_5$}  & $s_5$                     \\
\multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{$s_6$}  & $s_6$                      \\ \hline
\multicolumn{1}{l|}{$z_3$} & \multicolumn{1}{l|}{$z_2$} & \multicolumn{1}{l|}{$z_1$} & \multicolumn{1}{l}{$z_0$}
\end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
        %\caption{$P(x)$=$x^{4}+x+1$}
\begin{tabular}{cccc}
\multicolumn{4}{l}{$P(x)$=$x^{4}+x+1$}                                                                            \\
\multicolumn{1}{c|}{$s_3$} & \multicolumn{1}{c|}{$s_2$} & \multicolumn{1}{c|}{$s_1$} & $s_0$                     \\
\multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{$s_4$} & $s_4$                     \\
\multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{$s_5$}  & \multicolumn{1}{c|}{$s_5$}  & 0                     \\
\multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{0}  & 0                      \\ \hline
\multicolumn{1}{l|}{$z_3$} & \multicolumn{1}{l|}{$z_2$} & \multicolumn{1}{l|}{$z_1$} & \multicolumn{1}{l}{$z_0$}
\end{tabular}    \end{minipage} 
\caption{Analysis of the computation complexity of Galois field multipliers with different irreducible polynomials using two 4-bit GF multiplications, which are implemented using $x^{4}+x^{3}+1$ and $x^{4}+x+1$.}
\label{fig:study}
\end{figure}



==> date17-gf_example.tex <==


\begin{figure}[ht]
%\begin{table}[]
\small
\centering
\begin{tabular}{lllllll}
             &              &              & $a_3$        & $a_2$        & $a_1$        & $a_0$        \\
             &              &              & $b_3$        & $b_2$        & $b_1$        & $b_0$        \\ \hline
             &              &              & $a_{3}b_{0}$ & $a_{2}b_{0}$ & $a_{1}b_{0}$ & $a_{0}b_{0}$ \\
             &              & $a_{3}b_{1}$ & $a_{2}b_{1}$ & $a_{1}b_{1}$ & $a_{0}b_{1}$ &              \\
             & $a_{3}b_{2}$ & $a_{2}b_{2}$ & $a_{1}b_{2}$ & $a_{0}b_{2}$ &              &              \\
$a_{3}b_{3}$ & $a_{2}b_{3}$ & $a_{1}b_{3}$ & $a_{0}b_{3}$ &              &              &              \\ \hline
$s_6$        & $s_5$        & $s_4$        & $s_3$        & $s_2$        & $s_1$        & $s_0$       
\end{tabular}
\vspace{3mm}
%\caption{My caption}
\label{my-label}
%\end{table}
        \begin{minipage}{.5\linewidth}
      %\caption{$P(x)$=$x^{4}+x^{3}+1$}
      \centering
\begin{tabular}{cccc}
\multicolumn{4}{l}{$P(x)_{1}$=$x^{4}+x^{3}+1$}                                                                            \\
\multicolumn{1}{c|}{$s_3$} & \multicolumn{1}{c|}{$s_2$} & \multicolumn{1}{c|}{$s_1$} & $s_0$                     \\
\multicolumn{1}{c|}{$s_4$} & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{0} & $s_4$                     \\
\multicolumn{1}{c|}{$s_5$} & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{$s_5$}  & $s_5$                     \\
\multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{$s_6$}  & $s_6$                      \\ \hline
\multicolumn{1}{l|}{$z_3$} & \multicolumn{1}{l|}{$z_2$} & \multicolumn{1}{l|}{$z_1$} & \multicolumn{1}{l}{$z_0$}
\end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
        %\caption{$P(x)$=$x^{4}+x+1$}
\begin{tabular}{cccc}
\multicolumn{4}{l}{$P(x)_{2}$=$x^{4}+x+1$}                                                                            \\
\multicolumn{1}{c|}{$s_3$} & \multicolumn{1}{c|}{$s_2$} & \multicolumn{1}{c|}{$s_1$} & $s_0$                     \\
\multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{$s_4$} & $s_4$                     \\
\multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{$s_5$}  & \multicolumn{1}{c|}{$s_5$}  & 0                     \\
\multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{0}  & 0                      \\ \hline
\multicolumn{1}{l|}{$z_3$} & \multicolumn{1}{l|}{$z_2$} & \multicolumn{1}{l|}{$z_1$} & \multicolumn{1}{l}{$z_0$}
\end{tabular}    \end{minipage} 
\caption{\small Two GF($2^4$) multiplications constructed using $P(x)_{1}$=$x^{4}+x^{3}+1$ and $P(x)_{2}$=$x^{4}+x+1$.}
\vspace{-7mm}
\label{fig:4-bit-gf}
\end{figure}

==> systemc.tex <==
\begin{table}[]
\scriptsize
\centering
\label{tbl:systemC}
\begin{tabular}{|l|}
\hline
\begin{tabular}[c]{@{}l@{}}for (i = 0; i \textless 5; i++)\\ \{\\~~if(x $>$ y \&\& x $<$ 2*y)\\~~~~~ f = f - x; \\~~else\\~~~~~~f = f + y;\\ \}\end{tabular} \\ \hline
\end{tabular}
\caption{C++ implementation example}
\vspace{-3mm}
\end{table}

==> table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{My caption}
\label{my-label}
\begin{tabular}{|r|r|r|r|r|r|r|r|r|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\# of\\ Functions\end{tabular}}} & \multicolumn{2}{c|}{\textit{GF(2\textasciicircum 8)}} & \multicolumn{2}{c|}{\textit{GF(2\textasciicircum 64)}} & \multicolumn{2}{c|}{\textit{GF(2\textasciicircum 128)}} & \multicolumn{2}{c|}{\textit{GF(2\textasciicircum 256)}} \\ \cline{2-9} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{Area} & \multicolumn{1}{c|}{Delay} & \multicolumn{1}{c|}{Area} & \multicolumn{1}{c|}{Delay} & \multicolumn{1}{c|}{Area} & \multicolumn{1}{c|}{Delay} & \multicolumn{1}{c|}{Area} & \multicolumn{1}{c|}{Delay} \\ \hline
1 & 971 & 111.13 & 4.74e+04 & 175.01 & 1.89e+05 & 198.24 & 7.32e+05 & 224.14 \\ \hline
2 & 1243 & 136.84 & 4.97e+04 & 214.31 & 1.92e+05 & 228.10 & 7.37e+05 & 257.82 \\ \hline
4 & 1735 & 139.07 & 5.46e+04 & 208.25 & 1.97e+05 & 246.65 & 7.57e+05 & 272.10 \\ \hline
8 & 2786 & 148.64 & 6.20e+04 & 225.33 & 2.13e+05 & 250.31 & 7.90e+05 & 274.92 \\ \hline
16 & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & 7.60e+04 & 240.09 & 2.48e+05 & 259.37 & 8.50e+05 & 281.87 \\ \hline
\end{tabular}
\end{table}
